Thinking Broad, Acting Fast: Latent Reasoning Distillation from Multi-Perspective Chain-of-Thought for E-Commerce Relevance

Effective relevance modeling is crucial for e-commerce search, as it aligns search results with user intent and enhances customer experience. Recent work has leveraged large language models (LLMs) to address the limitations of traditional relevance models, especially for long-tail and ambiguous queries. By incorporating Chain-of-Thought (CoT) reasoning, these approaches improve both accuracy and interpretability through multi-step reasoning. However, two key limitations remain: (1) most existing approaches rely on single-perspective CoT reasoning, which fails to capture the multifaceted nature of e-commerce relevance (e.g., user intent vs. attribute-level matching vs. business-specific rules); and (2) although CoT-enhanced LLM's offer rich reasoning capabilities, their high inference latency necessitates knowledge distillation for real-time deployment, yet current distillation methods discard the CoT rationale structure at inference, using it as a transient auxiliary signal and forfeiting its reasoning utility. To address these challenges, we propose a novel framework that better exploits CoT semantics throughout the optimization pipeline. Specifically, the teacher model leverages Multi-Perspective CoT (MPCoT) to generate diverse rationales and combines Supervised Fine-Tuning (SFT) with Direct Preference Optimization (DPO) to construct a more robust reasoner. For distillation, we introduce Latent Reasoning Knowledge Distillation (LRKD), which endows a student model with a lightweight inference-time latent reasoning extractor, allowing efficient and low-latency internalization of the LLM's sophisticated reasoning capabilities. Evaluated in offline experiments and online A/B tests on an e-commerce search advertising platform serving tens of millions of users daily, our method delivers significant offline gains, showing clear benefits in both commercial performance and user experience.

==> Online_Evaluation.tex <==
\subsection{Online Evaluation}
We conducted a 7-day online A/B test on AliExpress’s search advertising system, assigning 10\% of user traffic to our distilled model with latent reasoning capability and 10\% to an equivalent student model without such reasoning components. In online deployment, the relevance model outputs a relevance score for each query–item pair, which is then assigned to a discrete numeric relevance level (e.g., 0 to 4, representing \textit{Irrelevant} to \textit{Exact}) based on predefined business rules and calibrated thresholds. Query-item pairs assigned to the low relevance tiers(e.g., tier 0 or 1) are filtered before the ranking module. Our approach achieved consistent and statistically significant improvements: +1.42\% in RPM, +0.48\% in CTR and +0.4\% in human-evaluated RS score. These gains confirm that our framework delivers more intent-aligned ads, enhances user experience, improves ad exposure efficiency, and ultimately boosts commercial performance in our search advertising pipeline.

% \subsubsection{Online Deployment}
%  For online deployment, our A/B test adopts a highly efficient 2-layer BERT-Tiny architecture augmented with the latent reasoning extractor, which is retained at inference time to enable reasoning-aware relevance scoring while meeting strict latency requirements of online serving. This model is trained using 400 million  annotations generated by the TOOD framework offline. During online serving, the model outputs the relevance score for each query--item pair. This score is then assigned to a discrete numeric relevance level (e.g., 0 to 4, representing \textit{Irrelevant} to \textit{Exact}) according to predefined business rules and calibrated thresholds. query-item pairs assigned to the low relevance tiers (e.g., tier 0 or 1) are filtered out before entering the ranking module. This pre-ranking filtering ensures that only ad items with sufficient semantic relevance to the user query are eligible for display in AliExpress search results, thereby improving both user experience and system efficiency.

% \subsubsection{Online Performance}
% We conducted an A/B test on AliExpress’s search advertising system to evaluate the effectiveness of our framework. A random 10\% of user traffic was assigned to the treatment group, which employed the TODO-based relevance model, while another 10\% served as the control group using the standard BERT-tiny model. To mitigate the impact of traffic fluctuations, the experiment was carried out for at least 7 consecutive days, with continuous monitoring of key performance indicators as following.
% \begin{itemize}
%     \item \textbf{RPM} (Revenue Per Mille): revenue generated per thousand ad impressions.
%     \item \textbf{CTR} (Click-Through Rate): ratio of ad clicks to impressions.
%     \item \textbf{COV} (Coverage): fraction of ads exposed to users, relative to the entire search page.
% \end{itemize}

% In addition, we measured \textbf{Relevance Satisfaction (RS)}, a human-evaluated metric that evaluates how well the displayed ads align with the user's search intent. Expert annotators reviewed approximately 3000 query--ad pairs from both groups to compute RS scores. As shown in Table~\ref{tab:online_results}, the TODO framework yields consistent and statistically significant improvements across all metrics:

% \begin{table}[h]
% \centering
% \caption{Online improvements of TODO on AliExpress.}
% \label{tab:online_results}
% \begin{tabular}{lcccc}
% \toprule
% Metric & RPM & CTR & COV & RS \\
% \midrule
% Improvement (\%) & +1.08 & +0.7 & +0.77 & +1.41 \\
% \bottomrule
% \end{tabular}
% \end{table}

% The results demonstrate that: (1) the notable gain in \textbf{RS} confirms that TODO delivers more intent-aligned ads; (2) the increase in \textbf{CTR} reflects higher user engagement due to improved relevance; (3) the rise in \textbf{COV} indicates that better relevance not only attracts clicks but also drives actual purchases; and (4) these combined effects lead to a measurable uplift in \textbf{RPM}. Overall, TODO enhances both user satisfaction and commercial performance in AliExpress’s search advertising system.

==> Related_Works.tex <==
\section{Related Works}
\subsection{Relevance Modeling for E-Commerce}
Relevance modeling is a core component of e-commerce search, which aims to estimate the semantic match between user queries and items. Early approaches relied on statistical methods like TF-IDF~\citep{ramos2003using} and BM25~\citep{robertson2009probabilistic}, which are efficient but limited in capturing deep semantic relationships. With the development of deep learning, neural methods have been applied in the relevance modeling task. The first wave involves learning dense representations for queries and items using the dual-encoder model \cite{10.1145/2505515.2505665,Palangi2014SemanticMW}, but their potential is constrained by the weak interaction between the query and item representations. This limitation was addressed by interaction-based models such as BERT\cite{kenton2019bert}, Colbert\citep{khattab2020colbert} and PolyEncoder \citep{humeaupoly}, which explore token-level interaction through cross-attention or dedicated interaction modules, yielding strong relevance performance in e-commerce search. Despite their success, bert-style models remain constrained on long-tail or ambiguous queries, motivating recent efforts to leverage Large Language Models (LLMs) for more robust and reasoning-aware relevance judgment.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{main.pdf}
    \caption{Framework overview of MPCoT teacher training (top) and LRKD student distillation and deployment (bottom).}
    \Description{Top: Multi-Perspective CoT (MPCoT) teacher training with SFT and cross-perspective DPO. Bottom: Student model with latent reasoning extractor—used during distillation (with CoT guidance loss) and retained for efficient online serving.}
    \label{fig:overall}
\end{figure*}

\subsection{LLM for Relevance}
Large Language Models (LLMs) have shown strong performance for e-commerce relevance via prompting or fine-tuning in recent works ~\cite{10.1145/3578337.3605136,yan2024consolidating,mehrdad2024large,wang2025llm}. However, treating LLMs as black-box annotators limits transparency and hinders advanced optimization (e.g., reinforcement learning~\cite{schulman2017proximal,rafailov2023direct}). To improve interpretability, recent approaches elicit Chain-of-Thought (CoT) alongside predictions~\cite{wei2022chain}. For example, \citet{Zhao_2025} models relevance as an interpretable CoT reasoning process and distills both rationales and score distributions from an explainable LLM to improve student models’ semantic interaction, while \citet{Tang_2025} employs a multi-stage SFT with diverse CoT strategies to guide the model in their LREF framework. Other works improve LLM reasoning via external signals or reinforcement learning, including incorporating user behavior~\cite{chen2025towards}, applying DPO to reduce optimistic bias~\cite{rafailov2023direct,Tang_2025}, or using GRPO to mitigate reasoning hallucinations~\cite{shao2024deepseekmath,dong_taosr1_2025}.  %However, these methods typically generate reasoning from a single perspective, potentially overlooking the multifaceted nature of relevance. In this paper, we address this by introducing a multi-perspective CoT framework that integrates diverse viewpoints to foster more comprehensive reasoning.

% \subsection{LLM for Relevance}
% Recent advances in Large Language Models (LLMs) \cite{achiam2023gpt,yang2025qwen3,guo2025deepseek} have shown to achieve performance superior to smaller models trained on extensive data, even in a few-shot setting. Consequently, a line of work has begun to explore the application of LLMs in relevance tasks \cite{10.1145/3578337.3605136,yan2024consolidating,mehrdad2024large,wang2025llm}. \citet{wang2025llm} demonstrated the downstream benefits of using fine-tuned LLMs as relevance annotators
% %, showing how their efficiency enables sophisticated sampling strategies that dramatically reduce the Minimum Detectable Effect (MDE) in online experiments
% . \citet{mehrdad2024large} systematically explored various fine-tuning techniques on a massive industrial dataset, enabling LLMs to reach a performance level on par with human annotators. \citet{yan2024consolidating} leverage LLM's superior pairwise ranking capabilities to correct and enhance its directly generated relevance scores, thereby producing higher-quality pseudo-labels. Despite these successes, the predominant use of LLMs as 'black-box' annotators introduces a critical challenge: a lack of transparency. This opacity not only undermines the explainability required for trustworthy systems but also precludes advanced optimization techniques, such as reinforcement learning \cite{schulman2017proximal,rafailov2023direct,shao2024deepseekmath} that depend on granular feedback into the model's reasoning process, thus limiting the upper bounds of performance.

% To address this, a growing body of research \cite{chen2025towards,Zhao_2025, Tang_2025} focuses on making the LLM's decision-making process more transparent by eliciting not only a relevance judgment but also the underlying reasoning, often through Chain-of-Thought (CoT) \cite{wei2022chain} methodologies. For example, \citet{Zhao_2025} propose to use a powerful open-source LLM to generate training data with explicit CoT reasoning steps, which is then used for the supervised fine-tuning of (SFT) a target LLM, enabling it to perform explainable relevance judgments. \citet{Tang_2025} introduced a more intricate multi-stage SFT framework, employing multiple CoT strategies to instill complex domain rules and reflective capabilities. Furthermore, recent works enhance LLM reasoning via external signals or reinforcement learning. For example, by incorporating user behavior~\cite{chen2025towards}, applying DPO to mitigate optimistic bias~\cite{rafailov2023direct}, or using Group Relative Policy Optimization (GRPO) \cite{shao2024deepseekmath} to address hallucination in reasoning~\cite{dong_taosr1_2025}. However, these methods typically generate reasoning from a singular perspective, potentially overlooking the multifaceted nature of relevance. In this paper, we address this by introducing a multi-perspective CoT framework that integrates diverse viewpoints (e.g., user vs. expert) to foster more comprehensive reasoning and enhance model performance.


% Furthermore, they apply Direct Preference Optimization (DPO) \cite{rafailov2023direct} to correct the model's inherent optimistic biases. Meanwhile, \citet{chen2025towards} augment the reasoning process with external knowledge through a behavior-augmented prompting method, where real-time user interaction data is retrieved to guide the LLM's step-by-step judgment.  \citet{dong_taosr1_2025} introduce an on-policy reinforcement learning stage that combines Group Relative Policy Optimization (GRPO) \cite{shao2024deepseekmath} with a difficulty-based dynamic sampling strategy to specifically mitigate the 'discriminative hallucination' problem, where the model produces a correct reasoning chain but an incorrect final label. 


\subsection{Knowledge Distillation for Relevance}
Knowledge Distillation (KD)~\cite{hinton2015distilling} is widely used to deploy large models in real-world search systems. Early work focused on compressing Transformer-based rankers (e.g., BERT) via score-based distillation~\cite{liu2022knowledge,reddi2021rankdistil,zhuang2021ensemble}, often using specialized losses like Margin-MSE~\cite{hofstatter2020improving}. With the rise of LLMs as powerful teachers, recent methods distill LLM-generated pseudo-labels into smaller models like BERT~\cite{ye2025best,shang2025knowledge,ye2025applying}. However, most treat the LLM as a black-box annotator, underutilizing its rich reasoning. A few recent works begin to distill Chain-of-Thoughts (CoTs): \citet{Zhao_2025} use token-level tagging to transfer attribute-level reasoning, while \citet{agrawal-etal-2025-rationale} train a decoder to reconstruct rationales as an auxiliary task. However, these methods discard rationales at inference, limiting the utility of the online environment.


% \subsection{Knowledge Distillation for Relevance}

% Knowledge Distillation (KD) \cite{hinton2015distilling} is a pivotal technique for deploying powerful but computationally expensive models in real-world search systems. Initially, KD in relevance modeling focused on compressing large Transformer-based rankers \cite{sun2023instruction} , such as distilling a BERT-base model into a smaller one \cite{liu2022knowledge,reddi2021rankdistil}, or distilling an ensemble of models into a single student to reduce inference costs \cite{zhuang2021ensemble}. These methods often employed specialized loss functions like Margin-MSE \cite{hofstatter2020improving} to accommodate the varying score distributions between different teacher and student architectures.

% More recently, with the advent of LLMs as superior teacher models, this paradigm has been extended to distill the ranking capabilities of LLMs into smaller models like BERT \cite{ye2025best}. These methods often utilize LLMs to generate pseudo-labels for large-scale unlabeled data \cite{shang2025knowledge}. \citet{ye2025applying} propose a hybrid distillation approach that combines Margin-MSE with KL-divergence to transfer both score and distribution knowledge, while also exploring using the LLM to generate hard negative samples. However, most existing distillation methods only scratch the surface of what LLMs can offer. They primarily treat the LLM as a data annotator and have not fully explored how to transfer its deeper, intrinsic knowledge. Specifically, the rich reasoning knowledge embedded in Chain-of-Thought (CoT) processes and the fine-grained relevance signals contained within the model's output probability distribution remain largely unexplored. \citet{Zhao_2025} propose a multi-dimensional knowledge distillation framework that first trains an LLM to produce structured CoT reasoning, and then transfers this knowledge through a multi-dimensional distillation process, where a student model learns the final score distribution while also learning to predict attribute-level matches from the CoT reasoning via an auxiliary sequence tagging task. \citet{agrawal-etal-2025-rationale} propose a rationale-guided distillation method using a cross-encoder-decoder student model. The encoder handles the primary classification task, while the decoder is trained to generate the LLM's rationale, with its generation loss serving as the auxiliary task to enhance the encoder's representations.




